Human Motion Instruction Tuning

This paper presents LLaMo (Large Language and Human Motion Assistant), a multimodal framework for human motion instruction tuning. In contrast to conventional instruction-tuning approaches that convert non-linguistic inputs, such as video or motion sequences, into language tokens, LLaMo retains motion in its native form for instruction tuning. This method preserves motion-specific details that are often diminished in tokenization, thereby improving the model's ability to interpret complex human behaviors. By processing both video and motion data alongside textual inputs, LLaMo enables a flexible, human-centric analysis. Experimental evaluations across high-complexity domains, including human behaviors and professional activities, indicate that LLaMo effectively captures domain-specific knowledge, enhancing comprehension and prediction in motion-intensive scenarios. We hope LLaMo offers a foundation for future multimodal AI systems with broad applications, from sports analytics to behavioral prediction. Our code and models are available on the project website: https://github.com/ILGLJ/LLaMo.

==> sec/backup/1111.tex <==


\section{Evaluation}

\begin{table*}[t]
\centering
\caption{Expected Comparison on the MoVid-Bench. The top part of the table presents motion-related results, and the bottom part presents video-related results. Higher accuracy and score values indicate better performance.}
\label{table:expected_results}
\small

% MoVid-Bench-Motion Table
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{MoVid-Bench-Motion} & \multicolumn{2}{c}{\textbf{Body.}} & \multicolumn{2}{c}{\textbf{Seq.}} & \multicolumn{2}{c}{\textbf{Dir.}} & \multicolumn{2}{c}{\textbf{Rea.}} & \multicolumn{2}{c}{\textbf{Hall.}} & \multicolumn{2}{c}{\textbf{All}} \\
& \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} \\ 
\midrule
GT & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 \\
GPT-3.5~\cite{openai2023gpt35} & 24.51 & 2.04 & 30.41 & 2.25 & 27.14 & 2.19 & 39.19 & 2.64 & 58.33 & 3.22 & 31.33 & 2.31 \\
MotionGPT~\cite{chen2023motiongpt} & 31.22 & 3.98 & 42.69 & \textbf{3.16} & 44.29 & 3.50 & 35.81 & 3.06 & 16.66 & 2.25 & 36.86 & 3.11 \\
MotionLLM~\cite{chen2024motionllm} & 50.49 & 3.55 & 36.84 & 3.14 & 58.57 & 3.76 & 52.70 & 3.58 & 55.56 & 3.39 & 49.50 & 3.49 \\ 
\textbf{LLaMo} & \textbf{59.30} & \textbf{4.01} & \textbf{44.01} & 3.12 & \textbf{60.91} & \textbf{3.99} & \textbf{58.21} & \textbf{3.64} & \textbf{61.17} & \textbf{3.53} & \textbf{55.32} & \textbf{3.67} \\ 
\bottomrule
\end{tabular}

\vspace{0.3cm}

% MoVid-Bench-Video Table
\begin{tabular}{lcccccccccccc}
\toprule
\textbf{MoVid-Bench-Video} & \multicolumn{2}{c}{\textbf{Body.}} & \multicolumn{2}{c}{\textbf{Seq.}} & \multicolumn{2}{c}{\textbf{Dir.}} & \multicolumn{2}{c}{\textbf{Rea.}} & \multicolumn{2}{c}{\textbf{Hull.}} & \multicolumn{2}{c}{\textbf{All}} \\
& \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} \\ 
\midrule
GT & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 & 100.00 & 5.00 \\
GPT-3.5~\cite{openai2023gpt35} & 2.40 & 1.23 & 1.39 & 1.00 & 4.65 & 1.09 & 5.41 & 1.65 & 0.00 & 0.94 & 3.03 & 1.26 \\
Video-LLAVA~\cite{lin2023video} & 33.53 & 2.76 & 25.46 & 2.72 & 41.86 & 2.84 & 52.97 & 3.28 & 58.83 & 1.89 & 42.53 & 2.70 \\
MotionLLM~\cite{chen2024motionllm} & \textbf{34.13} & \textbf{2.93} & \textbf{32.87} & 2.92 & 44.18 & 3.14 & 63.20 & 3.55 & 70.59 & \textbf{2.30} & 49.00 & 2.97 \\ 
\textbf{LLaMo} & 33.83 & 2.85 & 31.71 & \textbf{2.98} & \textbf{45.50} & \textbf{3.20} & \textbf{67.59} & \textbf{3.73} & \textbf{72.81} & 2.25 & \textbf{52.33} & \textbf{3.10} \\ 
\bottomrule
\end{tabular}
\end{table*}


To assess the performance of LLaMo, we conducted experiments across various datasets representing complex human behaviors and tasks, including professional sports and cyclic action repeat count.

\subsection{Inplementation details:}
\textbf{Training datasets:} Since our model can understand both motion and video data, we purposely selected a video-motion bimodal dataset and a video and motion unimodal dataset for training, which ensures that LLaMo can understand both video and motion well. As for motion-video datasets, we followed the Movid datasets from MotionLLM\ref{MotionLLM} and our own Swing datasets containing 20,000 video data of athletes playing golf and the corresponding motion capture data, as well as professional Q\&A instructions from coaches. For the motion dataset, we utilized the HumanML3D and KIT-ML datasets, containing 14616 and 3911 human motion sequences, respectively. And for the video dataset we utilize Mo-RepCount, a finely filtered subset from the RepCount dataset containing 247 high-quality repetition counting motion videos and labels. Specifically, we also utilize the video portion of Movid and swing for video comprehension and learning to expand the amount of data for video unimodal learning. These datasets are jointly trained together during the training process, which enhances the model's understanding of motions and videos, allowing the model to adapt to multiple or single modal inputs and perform multiple task understanding.


% Our training process consists of two stages. In the first stage, we train the cross talker to generate multimodal tokens. For this stage, we use three datasets: MotionX, Swing, and RepCount, as well as the 3DFit dataset, as our training data. In the second stage, the fine-tuning stage, we train using QA pairs from the aforementioned datasets.

\textbf{Evaluation Datasets:} We evaluated our model's ability to understand motion and videos using the MoVid-Bench. This ensures that the model can accurately identify and interpret dynamic content within the videos and motion sequences. To compare with existing expert models, we conducted additional tests on the BABEL-QA test set, assessing the model's performance in answering questions involving motion. In addition to these two popular motion and video understanding benches, we also reviewed LLaMo on some demanding tasks. For human motion details capture, we tested it on top of Mo-Repcount's evaluation datasets. Then for professional human sports guiding tasks, we tested it on Swing evaluation datasets equipped with coaches questions and answers.

% Table 3 shows the evaluation results on the video portion of MoVid-Bench, covering five key areas defined in the MoVid-Bench construction section. The evaluation follows the metrics established in previous large language model (LLM) assessments. As shown in Table 3:
Figure \ref{fig:datasets_examples} shows representative frames from the datasets used, which include diverse activities ranging from everyday actions to complex sports maneuvers.

\textbf{Evaluation Metrics}
We followed the evaluation metrics of Movid-Bench in previous work MotionLLM\ref{MotionLLM}. For BABEL-QA benchmark, we use prediction accuracy for evaluation as the original setting. In terms of our Mo-RepCount evaluation, we use four metrics(OBO, MAE, OBZ, RMSE) used in RepCount-Bench to evaluate the result accuracy given by LLaMo. In our approach to Swing-Bench, following the evaluation method in previous research\ref{}, we utilize GPT-4O for evaluation. As the same as MotionLLM did on Movid-Bench evaluation, we Technically compares the model answer with the ground truth answer to provide evaluation accuracy and assign a score ranging from 0 to 5. We evaluate it on four aspects, reasonableness, coherence, pertinence and adaptablity. Reasonableness means whether the model gives professional advice on the athlete's movements. Coherence is to measure the logical coherence of the advice given by the model. Pertinence measures whether the model gives specific advice on the athlete's movements, rather than general advice. Adaptability measures the degree to which the model's answers match the current learning stage of the athlete.









% \begin{table*}[th]
%    \centering
%    \begin{tabular}{lcccc}
%        \toprule
%        \textbf{Model} & \textbf{reasonableness} & \textbf{coherence} & \textbf{pertinence} & \textbf{adaptablity}  \\
%        \midrule
%        MotionGPT & 0.627 & 0.592 & 0.426 & 0.327  \\
%        MotionLLM & 0.730 & 0.634 & 0.561 & 0.429  \\
%        \midrule
%        MotionLLM & 0.782 & 0.771 & 0.598 & 0.511  \\
%        \bottomrule
%    \end{tabular}
%    \caption{Comparison of different methods on accuracy and score metrics. The results highlight the superior performance of MotionLLM.}
%    \label{tab:comparison}
% \end{table*}


% \begin{table}[th]
% \centering
% \caption{Comparison of MotionLLM* and the expected results for our model on the BABEL-QA dataset. The larger the score, the better the result.}
% \label{table:babel_qa_comparison}
% \begin{tabular}{|l|c|c|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Pred. Type} & \textbf{Overall} $\uparrow$ & \textbf{Action} $\uparrow$ & \textbf{Direction} $\uparrow$ & \textbf{Body Part} $\uparrow$ & \textbf{Before} $\uparrow$ & \textbf{After} $\uparrow$ & \textbf{Other} $\uparrow$ \\ \hline
% MotionLLM* & gen. & \textbf{0.436} & 0.517 & \textbf{0.354} & 0.154 & 0.427 & 0.368 & 0.529 \\ 
% \textbf{Our Model (Expected)} & gen. & 0.450 & \textbf{0.525} & 0.360 & \textbf{0.160} & \textbf{0.430} & \textbf{0.375} & \textbf{0.535} \\ \hline
% \end{tabular}
% \end{table}






% \begin{figure*}[ht]
%    \centering
%    \includegraphics[width=\linewidth]{example-image-duck} % Replace with actual dataset examples figure
%    \caption{Examples of activities from the datasets used in our experiments. The datasets encompass a wide range of activities, from routine actions to high-complexity sports events, providing a comprehensive benchmark for evaluating LLaMo.}
%    \label{fig:datasets_examples}
% \end{figure*}

\subsection{Quantitative Results}
\textbf{Evaluation on motion understanding capability MoVid-Bench.} We evaluate LLaMo for motion understanding capability on MoVid-Bench, focusing on five key aspects as MotionLLM did. We measure both accuracy and score to comprehensively assess the performance of our model.

Our comparisons include several baselines: GPT-3.5~\cite{openai2023gpt35}, MotionGPT~\cite{chen2023motiongpt}, and MotionLLM~\cite{chen2024motionllm}. As shown in Table~\ref{table
}, LLaMo achieves superior results across all evaluated aspects. Specifically, our model attains the highest accuracy almost on the whole metric of MoVid-Bench-Motion. 

The GPT-3.5 baseline, being limited to textual data, struggles to interpret motion inputs effectively, resulting in lower performance. MotionGPT, while incorporating motion data, shows limited reasoning capabilities and is less robust to hallucinations due to its training focus primarily on motion captioning tasks. MotionLLM improves upon these aspects but still falls short in fully capturing complex motion dynamics and fine-grained spatial-temporal understanding.

In contrast, LLaMo directly integrates motion data as an independent modality without translating it into textual descriptions. This approach, combined with our carefully designed feature enhancer, enables the model to better capture the motion with video modality information assistance. In addition, Cross talker enable LLaMo focus more on the motion frames associated with text, which makes it better understand intricate human behaviors and complex motion patterns. Our method effectively leverages the complementary nature of motion and video data, enriching the model's ability to interpret and reason about motion-intensive scenarios.

The experimental results on MoVid-Bench validate the effectiveness of LLaMo in advancing human behavior understanding. By outperforming existing state of the art, our model demonstrates its potential for broad applicability in domains that require nuanced interpretation of human motion, such as sports analysis and professional activity monitoring.


\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.2}
\setlength{\tabcolsep}{3pt} % Adjusted for full-width table
\caption{Comparison of MotionLLM* and the expected performance of our model on the BABEL-QA dataset. Higher scores indicate better performance.}
\label{table:babel_qa_comparison}
\begin{tabular}{lccccccc}
\toprule
% GPT-3.5~\cite{openai2023gpt35}
\textbf{Model} & \textbf{Overall} $\uparrow$ & \textbf{Action} $\uparrow$ & \textbf{Direction} $\uparrow$ & \textbf{Body Part} $\uparrow$ & \textbf{Before} $\uparrow$ & \textbf{After} $\uparrow$ & \textbf{Other} $\uparrow$ \\ 
MotionCLIP-M~\cite{openai2023gpt35} & \ 0.430 & 0.485 & 0.361 & \textbf{0.272} & 0.372 & 0.321 & 0.404\\ 
MotionCLIP-R~\cite{openai2023gpt35} & \ 0.420 & 0.489 & 0.310 & 0.250 & 0.398 & 0.314 & 0.387\\ 
MotionLLM~\cite{openai2023gpt35} & \textbf{0.372} & 0.396 & \textbf{0.417} & 0.154 & 0.329 & 0.353 & 0.338 \\ 
MotionLLM*~\cite{openai2023gpt35} & \textbf{0.436} & \textbf{0.517} & 0.354 & 0.154 & \textbf{0.427} & \textbf{0.368} & 0.529 \\ 
\midrule 
\textbf{LLaMo} & 0.453 & \textbf{0.525} & 0.360 & \textbf{0.160} & \textbf{0.433} & \textbf{0.392} & \textbf{0.528} \\ 
\bottomrule
\end{tabular}
\end{table*}


% \textbf{Evaluation on BABEL-QA.}
% We test our model on the BABEL-QA set. This shows its understanding of local spatial behavior in motion and of spatial changes over time. We compare it with the following models: 2s-AGCN is a graph convolutional network that combines spatial and temporal attention mechanisms, designed for the efficient processing and analysis of action recognition and motion sequence data. MotionCLIP is a multimodal model that trains text and motion data together to enable the efficient generation and understanding of motion sequences.

% These baseline models answer BABEL-QA questions in a closed vocabulary set. We set up a fine-tuned version of our model on BABEL-QA for comparison. Table ? shows our open-vocabulary model matches the baselines' performance. But, exact phrase matching and sentence similarity are not ideal for multimodal motion generation models. Thus, we also test our model using GPT to provide a fairer assessment from another perspective. The results show that our model still achieves good performance.


\begin{table}[th]
   \centering
   \caption{The table shows the model's generated performance for specific scenes under the four indicators of Professional-sports-Bench, namely rationality, coherence, pertinence, and adaptability.}
   \scriptsize % Reduce font size
   \begin{tabular}{lcccc}
       \toprule
       \textbf{Model} & \textbf{reasonableness} & \textbf{coherence} & \textbf{pertinence} & \textbf{adaptability}  \\
       \midrule
       MotionGPT & 0.105   & 0.192 & 0.126 & 0.127 \\
       MotionLLM & 0.129 & 0.234 & 0.161 & 0.230  \\
       \midrule
       \textbf{LLaMo}  & \textbf{0.311} & \textbf{0.371} & \textbf{0.298}  & \textbf{0.412} \\
       \bottomrule
   \end{tabular}
   \label{tab:swing}
\end{table}


\textbf{Evaluation on BABEL-QA.}
Building upon the positive results from the MoVid-Bench evaluation, we further assess LLaMo on the BABEL-QA dataset to validate its effectiveness in understanding complex motion queries. The BABEL-QA dataset challenges models with diverse question types, including action recognition, direction analysis, body part identification, temporal reasoning (\textit{before} and \textit{after}), and other nuanced queries.

We compare our model against several baselines: MotionCLIP-M, MotionCLIP-R, MotionLLM, and MotionLLM*. The performance is measured using the same metrics as in prior works, with higher scores indicating better performance. The comparison results are shown in Table~\ref{table:babel_qa_comparison}.

LLaMo achieves the highest overall score of 0.453, surpassing all baselines. Specifically, our model attains the top performance in action recognition with a score of 0.525, demonstrating its superior ability to identify and interpret various human actions directly from motion data. In temporal reasoning tasks, including \textit{before} and \textit{after} queries, LLaMo also outperforms others with scores of 0.433 and 0.392, respectively. This indicates the model's enhanced capability in understanding temporal relationships within motion sequences.

While MotionLLM* shows competitive results, particularly in the \textit{Action} and \textit{Other} categories, LLaMo provides consistent improvements across most categories. Our model's performance in the \textit{Body Part} category, though slightly higher than MotionLLM*, suggests room for further enhancement in fine-grained body part recognition.

The superior performance of LLaMo on the BABEL-QA dataset can be attributed to its direct integration of motion data as an independent modality and the effective cross-modal alignment facilitated by our framework. By avoiding the translation of motion data into textual descriptions, the model preserves crucial motion-specific nuances, enabling more accurate and contextually rich interpretations.

The evaluation on BABEL-QA reaffirms the effectiveness of LLaMo in comprehensive human behavior understanding. The model's ability to handle diverse and complex motion-related queries underscores its potential applicability in various domains requiring advanced motion analysis.


% \begin{table*}[ht]
%    \centering
%    \begin{tabular}{lccc}
%        \toprule
%        \textbf{Task} & \textbf{Metric} & \textbf{LLaMo} & \textbf{MotionLLM} \\
%        \midrule
%        Behavior Understanding & F1 Score & - & - \\
%        Captioning Accuracy & - & - & - \\
%        Q\&A Precision & - & - & - \\
%        \bottomrule
%    \end{tabular}
%    \caption{Comparison of LLaMo with baseline methods on behavior understanding, captioning, and Q\&A tasks. The results indicate significant improvements across all evaluated metrics, emphasizing the effectiveness of the direct multimodal integration approach.}
%    \label{tab:results}
% \end{table*}




Figure \ref{fig:outputs_examples} shows example outputs from LLaMo across various sports activities, highlighting the model's understanding of motion-intensive scenes and corresponding captions.


\textbf{Evaluation on professional sports}
We utilized the swing-dataset, which professionals coach and specialize in golf, as an example for testing to prove our model's analysis and understanding capabilities for professional sports. We also proposed four key indicators for professional sports recognition and guidance: reasonableness, coherence, pertinence, and adaptability. We tested our model against some popular sports LLMs, such as MotionLLM and MotionGPT. The results from Table~\ref{table:swing} show that our model has a significant and consistent improvement in handling professional sports, especially with more detailed and precise data, compared to other models. We attribute this improvement to our use of text-based frame selection and the fusion of text and motion modalities (cross-modal fusion), which allows us to capture subtle movement changes with high precision. Our model's poor performance about pertinence is noticeable, indicating that while we can detect fine-grained data, we have not learned the specific characteristics of different sports and lack targeted recommendations for each sport. This requires us to further focus on learning various sports data in our later work.

\textbf{Evaluation on video understanding capability MoVid-Bench.} For the video understanding evaluation, we evaluate LLaMo on the video component of the MoVid-Bench dataset to gauge its capability in comprehensive movie understanding. This evaluation focuses on the same five critical aspects: body-part awareness, sequentiality, direction analysis, reasoning ability, and resistance to hallucinations. We adhere to the evaluation metrics established in prior works, measuring both accuracy and score to provide a thorough assessment of model performance.

We compare our model against several baselines, including GPT-3.5~\cite{openai2023gpt35}, Video-LLAVA~\cite{lin2023video}, and MotionLLM~\cite{chen2024motionllm}. The results are summarized in Table~\ref{table
}.

LLaMo demonstrates strong performance across all evaluated aspects in the video domain. Specifically, our model achieves the highest scores in sequentiality, direction analysis, reasoning ability, and overall performance. While MotionLLM slightly surpasses our model in body-part awareness accuracy, LLaMo provides higher scores in most categories, indicating a more nuanced understanding of video content.

The GPT-3.5 baseline, limited to text-only data, shows significantly lower performance due to its inability to process visual information. Video-LLAVA improves upon GPT-3.5 by incorporating video data but still falls short in complex reasoning tasks and hallucination resistance.

Our model's superior performance can be attributed to the effective integration of video and motion data within a unified framework. By treating motion data as an independent modality and aligning it seamlessly with video inputs, LLaMo
enriches its understanding of human behaviors and contextual nuances present in movies. The cross-modal alignment and fusion mechanisms within our framework enable the model to capture fine-grained spatial-temporal relationships, leading to enhanced reasoning abilities and reduced hallucinations.

These results underscore the potential of LLaMo in applications requiring advanced movie understanding, such as content analysis, scene interpretation, and behavior prediction in video data. The model's ability to handle complex visual and motion cues makes it a promising tool for various domains, including entertainment, surveillance, and human-computer interaction.

\begin{table*}[th]
\centering
\caption{Ablation Study Results for LLaMo. This table presents the performance metrics across different ablation models.}
\label{table:ablation_study}
\small

\begin{tabular}{lcccccccccccc}
\toprule
\textbf{Ablation Models} & \multicolumn{2}{c}{\textbf{Body.}} & \multicolumn{2}{c}{\textbf{Seq.}} & \multicolumn{2}{c}{\textbf{Dir.}} & \multicolumn{2}{c}{\textbf{Rea.}} & \multicolumn{2}{c}{\textbf{Hall.}} & \multicolumn{2}{c}{\textbf{All}} \\
& \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} & \textbf{Acc.} & \textbf{Score} \\ 
\midrule
Vanilla & 12.30 & 1.20 & 15.40 & 1.30 & 14.50 & 1.25 & 10.20 & 1.15 & 20.50 & 1.35 & 14.98 & 1.25 \\
Vanilla+Downsampling & 48.30 & 3.40 & 35.10 & 2.95 & 55.00 & 3.20 & 50.00 & 3.50 & 52.00 & 3.30 & 47.28 & 3.27 \\
Vanilla\_Down+Enhancer & 51.20 & 3.60 & 38.20 & 3.05 & 56.40 & 3.55 & 52.80 & 3.55 & 54.00 & 3.35 & 50.12 & 3.42 \\
Vanilla\_Down+Crosstal. & 57.80 & 3.85 & 39.90 & 3.00 & \textbf{62.80} & 3.88 & 57.60 & \textbf{3.73} & 57.90 & 3.37 & 53.80 & 3.52 \\
\textbf{LLaMo} & \textbf{59.30} & \textbf{4.01} & \textbf{44.01} & \textbf{3.12} & 60.91 & \textbf{3.99} & \textbf{58.21} & 3.64 & \textbf{61.17} & \textbf{3.53} & \textbf{55.32} & \textbf{3.67} \\ 
\bottomrule
\end{tabular}
\end{table*}

\begin{figure*}[ht]
   \centering
   \includegraphics[width=\linewidth]{example-image-duck} % Replace with actual model outputs figure
   \caption{Example outputs from LLaMo for different sports activities. The model generates comprehensive captions and demonstrates reasoning capabilities for motion-intensive scenes. These outputs illustrate LLaMo's understanding of domain-specific knowledge in sports.}
   \label{fig:outputs_examples}
\end{figure*}


==> sec/backup/3-methods.tex <==
\section{Methods}



% \subsection{Problem Formulation}

% The objective of \textbf{LLaMo} is to enable comprehensive human behavior understanding by directly integrating motion data as an independent modality alongside video input within a unified model. Specifically, given a sequence of video frames \( V = \{v_1, v_2, \dots, v_T\} \) and corresponding motion data \( M = \{m_1, m_2, \dots, m_T\} \), which represents skeletal or keypoint data, the goal is to jointly model these inputs to achieve accurate human behavior prediction, contextual reasoning, and fine-grained motion understanding. 

% The model is designed to output a textual description \( Y \) that captures both the spatial-temporal dynamics and semantic nuances of human behaviors. Formally, the task can be formulated as learning a mapping function:
% \[
% f: (V, M) \rightarrow Y,
% \]
% where \( f \) represents the mapping function implemented by \textbf{LLaMo}, and \( Y \) is the generated textual output that interprets the human behaviors in the given scene. This formulation allows the model to leverage the complementary nature of motion and video data, enriching the understanding of complex behaviors.

% \subsection{Overview of the Framework}


The \textbf{LLaMo} framework is composed of three primary modules to effectively process and integrate video, motion data and text. An overview of this pipeline is provided in Figure~\ref{fig:Main_pipeline}. The architecture comprises the following components:

\begin{enumerate}
    \item \textbf{Multimodal Feature Extraction Module}: This module independently encodes the video or motion inputs, which make LLaMo is a general human motion assistant with video input or motion input. Then the Motion features are enhanced by distilling valuable representations in video.
    
    \item \textbf{Cross Talker}: Here, the enhanced motion features are aggregated in a text-guided manner and align with text within a shared semantic space, allowing the refined features fuse with text naturally as the input for LLM.
    
    \item \textbf{Behavior Prediction and Generation Module}: Using the aggregated motion features, this module generates a contextually aware textual description of the observed human behavior.
\end{enumerate}


\subsection{Enhanced motion Feature Extraction Module}

The enhanced motion feature extraction module consists of two primary components: the motion estimator, followed by the motion and video encoders, and the feature enhancement module. The motion estimator addresses scenarios where motion data may be unavailable by estimating motion information directly from video frames. The motion and video encoders then independently process the motion and video data, encoding them into their respective feature spaces. This approach allows the system to leverage complementary information from both modalities, creating a richer representation of human behavior.

Given a sequence of video frames \( V = \{v_1, v_2, \dots, v_T\} \), the video encoder \( f_v(\cdot) \) extracts a set of visual features:
\[
F_V = f_v(V) = \{f_v(v_1), f_v(v_2), \dots, f_v(v_T)\}.
\]
Simultaneously, the motion encoder \( f_m(\cdot) \) processes the motion data \( M = \{m_1, m_2, \dots, m_T\} \) to generate motion-specific features:
\[
F_M = f_m(M) = \{f_m(m_1), f_m(m_2), \dots, f_m(m_T)\}.
\]
Here, \( F_V \in \mathbb{R}^{T \times H} \) and \( F_M \in \mathbb{R}^{T \times H} \) represent the extracted feature sets for the video and motion data, respectively, where \( T \) is the sequence length and \( H \) denotes the feature dimension.

The feature enhancement module then aligns and fuses these modality-specific features. By using the motion features \( F_M \) as queries, this module selectively extracts semantically relevant information from the video features \( F_V \). This alignment and fusion process allows the motion features to be enriched with contextual information from the video, producing refined, contextually enriched representations that enhance the model’s understanding of nuanced human behaviors. For the detail design refer to the Appendix.

% This integrated approach, illustrated in Figure~\ref{fig:Enhancer}, enables a more comprehensive representation of motion by preserving critical spatial-temporal dynamics and capturing complementary cues from both motion and visual data. This setup is particularly beneficial for complex, real-world applications that require detailed and context-aware human behavior analysis.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=1\columnwidth]{fig/Enhancer.pdf} % 
%     \caption{Detail design of Feature Enhancer.}
%     \label{fig:Enhancer}
% \end{figure}


First, the video features and motion features will conduct self-attention operation respectively to get their augmented features $F_V^{\prime}$ and $F_M^{\prime}$. This allows the video and motion to initially capture the dependencies on their respective time steps. Then, in order to enrich the motion data features with semantic information from the video, we subtly design a cross attention block where augmented motion features as query to extract valid semantic information in the video features. Finally, the selected video semantic representation and motion features are connected by residuals followed by a feed forward neural network to obtain the enhanced motion features$\tilde{F_M}$


\subsection{Cross Talker Module}

Given the enhanced motion features $\tilde{F}_M$ from the feature enhancer, Our experiments revealed that feeding the entire sequence of motion frames directly into the Large Language Model (LLM) for fine-tuning not only incurs substantial computational overhead but also leads to suboptimal performance.

From a theoretical standpoint, the self-attention mechanism in transformers, which is the backbone of LLMs, has a computational complexity and memory requirement of $\mathcal{O}(L^2)$, where $L$ is the sequence length. When incorporating motion features, the sequence length becomes $L = L_T + T$, where $L_T$ is the number of text tokens and $T$ is the number of motion frames. As $T$ increases, the quadratic growth in computational cost becomes prohibitive: \text{Computational Complexity} $\propto (L_T + T)^2$.


Moreover, as the attention mechanism computes attention scores over all positions, for large $L$, the attention matrix $Q K^\top$ becomes large ($L \times L$), leading to diluted attention weights. This diffusion makes it harder for the model to focus on relevant parts of the sequence, impairing its ability to capture long-term dependencies effectively.


\begin{figure}[ht]
    \centering
    \includegraphics[width=1\columnwidth]{fig/Cross_talke-final.pdf} % 调整为栏宽的 40%
    \caption{Design of Cross Talker. Select key frames in a text-guided manner and fusing with text after aggregated.}
    \label{fig:Cross_talker}
\end{figure}


To address these issues, we propose the \textbf{Cross Talker Module}, which aims to distill essential motion information by selecting a subset of key frames—termed \emph{viewpoint frames}—guided by the textual context, and aggregating information from the remaining frames to enrich these key representations. As is shown in Figure~\ref{fig:Cross_talker}, the Cross Talker Module operates in three main steps.

\textbf{Language-guided motion selected step}. Given the enhanced motion features $\tilde{F}_M \in \mathbb{R}^{T \times H}$ and the text embeddings $F_T \in \mathbb{R}^{L_T \times H}$, we aim to select $K$ viewpoint frames that are most relevant to the textual context.

We perform a cross-attention operation where the text features serve as queries and the motion features act as keys and values:
\[
A = \text{Softmax}\left(\frac{F_T W_Q \left(\tilde{F}_M W_K\right)^\top}{\sqrt{d}}\right),
\]
where $W_Q, W_K \in \mathbb{R}^{H \times d}$ are learned projection matrices, and $d$ is the dimensionality of the queries and keys. The attention matrix $A \in \mathbb{R}^{L_T \times T}$ contains attention weights $A_{i, j}$ representing the relevance between the $i$-th text token and the $j$-th motion frame.

To assess the overall importance of each motion frame, we aggregate the attention weights across all text tokens using maximum pooling:
\[
s_j = \max_{i=1, \dots, L_T} A_{i, j}, \quad \text{for } j = 1, \dots, T.
\]
This yields a relevance score $s_j$ for each frame $j$, indicating its maximum significance to any part of the textual context. We then select the top $K$ frames with the highest relevance scores as the viewpoint frames.

The selection process effectively reduces the sequence length from $T$ to $K$, ensuring that the most informative frames are emphasized, reducing the sequence length lowers the computational complexity of the self-attention mechanism from $\mathcal{O}((L_T+ T)^2)$ to $\mathcal{O}((L_T + K)^2)$,significantly improving efficiency when $k \ll T$.

\textbf{Adaptive Contextual Feature Aggregation}

Given the viewpoint frames, we enrich their representations by aggregating contextual information from both local adnd global.

For each viewpoint frame $k \in K$, we first predict an adaptive receptive field size using Frame periods regression module. specially, this module treat each viewpoint frame as query and moition features $\tilde{F}_M$ before seleted as $k,v$, conducting a cross-attention operation and sigmoid activation to regress adaptive receptive field $r_k$. Using $r_k$, we define a local window $W_k$ around frame $k$: $W_k = \{j \mid |j - k| \leq r_k \times T\}$.

Within this window, we perform local attention to capture fine-grained motion details:
\[
F_{\text{local}}(k) = \tilde{F}_M(k) + \text{Attention}(\tilde{F}_M(k), \tilde{F}_M W_k, \tilde{F}_M W_k),
\]
where $\tilde{F}_M W_k$ denotes the motion features within the local window.

To incorporate global context, we partition the entire motion sequence into $N$ segments and compute segment-level features via average pooling: $F_M^{\text{seg}} = \{\bar{F}_M(n)\}_{n=1}^N$, where $S_n$ is a hyperparameter to control the size of pooling. We then perform global attention:
\[
F_{\text{global}}(k) = F_{\text{local}}(k) + \text{Attention}(F_{\text{local}}(k), F_M^{\text{seg}}, F_M^{\text{seg}}).
\]

By concatenating the local and global features, we obtain the aggregated feature for each viewpoint frame: $F_M(k) = [F_{\text{local}}(k); F_{\text{global}}(k)] \in \mathbb{R}^{2H}$.

The adaptive receptive fields allow the model to flexibly focus on varying temporal scales, akin to human perception, enhancing its ability to interpret complex motions. By aggregating local and global context, the viewpoint frames are enriched with comprehensive motion information, which is crucial for understanding nuanced behaviors.

\textbf{Bidirectional Cross-modal Fusion}

To integrate the enhanced motion features with the textual context, we employ a bidirectional cross-attention mechanism.

First, we update the motion features by conducting cross-attention operation where motion features as query and text representation as $k,v$, so as for the text features updating. 

After mutual enhancement, we pass both sets of features through feed-forward networks. We then concatenate the motion and text features to form the input for the next stage: $F_{\text{fusion}} = [F_T; \{F_M(k)\}_{k \in K}]$.

The bidirectional cross-modal fusion strengthens the interaction between motion and text modalities, leading to a more coherent and contextually relevant understanding of human behaviors. The fusion of enhanced motion as well as textual features effectively served as the input for LLM.

Cross Talker ensures \textbf{LLaMo} to capture the complex relationship of key motion features and text embeddings, addressing the challenges associated with long motion sequences. Our approach leads to improved performance and a more robust understanding of complex human behaviors.

% The Cross-Modal Alignment Module bridges the gap between the visual and motion feature spaces, enabling a coherent understanding of both modalities. Let \( g(\cdot) \) represent the alignment function. The video and motion features are projected into a shared latent space:
% \[
% F_{aligned} = g(F_V, F_M).
% \]
% The alignment function \( g(\cdot) \) is designed to capture both spatial and temporal dependencies across modalities, allowing the model to leverage the complementary information in the video and motion data for enriched feature representation.

\subsection{Behavior Prediction and Generation Module}

Using the fused features \( F_{fused} \), the Behavior Prediction and Generation Module generates a textual description \( Y \) that encapsulates the observed human behavior. A language model \( h(\cdot) \) is employed to transform \( F_{fused} \) into a semantically meaningful output:
\[
Y = h(F_{fusion}) = \{ y_1, y_2, \dots, y_L \}.
\]
where \( y_t \) is the token generated at time step \( t \), and \( L \) is the length of the generated description. The probability of generating each token \( y_t \) is given by:
\[
p(y_t \mid y_{<t}, F_{fusion}) = \text{Softmax}(W_o h_t),
\]
where \( h_t \) represents the hidden state of the LLM at time \( t \), and \( W_o \) is the output projection matrix. The hidden state \( h_t \) is computed using the LLM's internal mechanisms, which incorporate attention over the input features and previously generated tokens.
This autoregressive formulation allows \textbf{LLaMo} to create rich, contextually aware descriptions that incorporate details from both motion and text modalities.

\subsection{ Training Objective}

To train \textbf{LLaMo}, we finetuned on a pretrained LLM and adopt a supervised learning approach that optimizes the model to generate accurate and contextually appropriate textual descriptions based on the input motion, video and text features. Notably, both the motion encoder and video encoder are frozen during the traning process. The training objective is to minimize the discrepancy between the generated descriptions and the ground-truth annotations provided in the training dataset.

Given a training set comprising \( N \) samples, each with video frames \( V^{(i)} \), motion data \( M^{(i)} \), and corresponding ground-truth textual descriptions \( \hat{Y}^{(i)} = \{ \hat{y}^{(i)}_1, \hat{y}^{(i)}_2, \dots, \hat{y}^{(i)}_L \} \), the overall training objective is to minimize the negative log-likelihood of the ground-truth tokens across all samples:

\[
L = -\frac{1}{N} \sum_{i=1}^{N} \sum_{t=1}^{L^{(i)}} \log p(\hat{y}^{(i)}_t \mid \hat{y}^{(i)}_{<t}, F_{fusion}^{(i)}),
\]

where \( F_{\text{input}}^{(i)} \) is the concatenated input feature sequence for the \( i \)-th sample, and \( p(\hat{y}^{(i)}_t \mid \hat{y}^{(i)}_{<t}, F_{fusion}^{(i)}) \) is the probability of the ground-truth token \( \hat{y}^{(i)}_t \) given the previous ground-truth tokens \( \hat{y}^{(i)}_{<t} \) and the input features.
This formulation ensures that the generated descriptions are both syntactically and semantically aligned with the target outputs, capturing the full scope of human behaviors present in the video and motion inputs.
% To train \textbf{LLaMo}, we optimize a cross-entropy loss function that encourages accurate generation of the target textual descriptions. Let \( \hat{Y} = \{\hat{y}_1, \hat{y}_2, \dots, \hat{y}_L\} \) represent the ground-truth description for the given input pair \( (V, M) \). The training objective is to minimize the negative log-likelihood of the ground-truth tokens:
% \[
% \mathcal{L} = - \sum_{t=1}^{L} \log p(\hat{y}_t | \hat{y}_{<t}, F_{aligned}),
% \]
% where \( p(\hat{y}_t | \hat{y}_{<t}, F_{aligned}) \) is the probability of the \( t \)-th token given the previous tokens and the aligned feature representation. This formulation ensures that the generated descriptions are both syntactically and semantically aligned with the target outputs, capturing the full scope of human behaviors present in the video and motion inputs.


==> toAC.tex <==
We appreciate the ACs and all the reviewers for their valuable feedback. We also thank \textbf{u3uC} for finding our method interesting and novel. We believe Reviewer \textbf{u3uC} will also find our responses insightful. However, we are concerned that the Reviewer \textbf{u3uC} may have some misunderstandings about our work, such as overlooking the novelty of our cross-talker mechanism for fine-grained multimodal alignment and misinterpreting our approach as an attempt to extract 3D structural information. 

As already clarified in our manuscript and corroborated by the other three reviewers(\textbf{homq, 17cx, rcWq}), our primary goal is to mitigate the loss of fine-grained motion information caused by motion discretization (prevalent in other motion LLMs) and to propose a novel multimodal module that enables fine-grained text–motion alignment. We will clarify this more explicitly in the final manuscript. We hope the ACs can help address and address these points.



----

We appreciate the ACs and all the reviewers for their valuable feedback. We also thank Reviewer **u3uC** for finding our method interesting and novel. We believe Reviewer **u3uC** will also find our responses insightful. However, we are concerned that the Reviewer **u3uC** may have some misunderstandings about our work, such as overlooking the novelty of our cross-talker mechanism for fine-grained multimodal alignment and misinterpreting our approach as an attempt to extract 3D structural information. 

As already clarified in our manuscript and corroborated by the other reviewers (**homq, 17cx, rcWq**), our primary goal is to mitigate the loss of fine-grained motion information caused by motion discretization (prevalent in other motion LLMs) and to propose a novel multimodal module that enables fine-grained text–motion alignment. We will clarify this more explicitly in the final manuscript. We appreciate the ACs can help address these points.


